On Automating Conversations

From 2016 to 2018, we developed and deployed Chorus, a system that blends real-time human computation with artificial intelligence (AI) and has real-world, open conversations with users. We took a top-down approach that started with a working crowd-powered system, Chorus, and then created a framework, Evorus, that enables Chorus to automate itself over time. Over our two-year deployment, more than 420 users talked with Chorus, having over 2,200 conversation sessions. This line of work demonstrated how a crowd-powered conversational assistant can be automated over time, and more importantly, how such a system can be deployed to talk with real users to help them with their everyday tasks. This position paper discusses two sets of challenges that we explored during the development and deployment of Chorus and Evorus: the challenges that come from being an "agent" and those that arise from the subset of conversations that are more difficult to automate.

==> context.tex <==


\section{Data Preparation} \label{frame}
%Due to the modular nature of \system, we separately train the model in
%two stages with additional datasets, as described below.
\paragraph{Visual Genome}

This dataset contains labels for tasks in language and vision fields such as
object detection and object relation detection. Visual
Genome has 108,077 images, 3.8 million object instances, and 2.3 million
relationships.  We use it to pretrain the object detection model. In addition, 
we utilize the noun and verb relations provided by the scene graph of
Visual Genome 
% to ``kopfkino'' the possible activities which could link two photos.
to brainstorm activities which could link two photos.   
Relations of nouns and verbs in each image have been labeled as \textit{(subject, verb, object)}. 
We use verb relations for two reasons. 
First, compared to unseen objects,
activities are better additions to visual stories for correlation
as they do less harm to grounding. Second, as most image-to-text datasets focus
on objects, stories generated based on objects are relatively static. Hence adding
activities makes our stories more vivid.  


\paragraph{VIST Dataset}
%\lwku{for plot term extraction \& finetune generated story} 
This is a collection of 20,211 human-written visual stories and 81,743 unique photos.
Each story in VIST contains five sentences and five corresponding photo images.
To train our image-to-term prediction model, we first extract terms from
sentences of stories in the VIST dataset as the gold labels.
Inspired by Semstyle~\cite{Alexander2018Semstyle}, we consider the key components of a
sentence to be its noun (object) and verb (action) terms; 
%these terms are
%required in story generation as they provide the most essential information.
therefore, given a sentence, we first detect nouns and verbs using a
part-of-speech tagger.\footnote{SpaCy: https://spacy.io/} Then, we extract verb
frames to replace the original verbs using Open-SESAME~\cite{swayamdipta17open}, a
frame-semantic parser which automatically detects
FrameNet~\cite{baker1998berkeley} frames. For example,
%in Table~\ref{tab:term_example}
the terms extracted from \emph{``The dog is ready to go.''} are ``Dog\_Noun'' and ``Motion\_Frame''.


\paragraph{ROCStories Corpora} 
To train the story generator, we use the ROCStories
Corpora~\cite{mostafazadeh2016roc}, which contains 98,159 stories. As the
annotators of ROCStories were asked to write a five-sentence story given a
prompt, stories focus on a specific topic with strong logical
inference. As with VIST, we extract terms from sentences of stories which
are used as the input data for the story generation model.




\section{Experiments and Results}




==> data.tex <==
\subsection{Data Preparation}
Four datasets were used in this paper: Visual Genome, OpenIE, ROCStories Corpora,
and VIST Dataset.
VIST Dataset provides image-to-term materials for learning in Stage 1, and the
object relations from Visual Genome together with the term relations from OpenIE are
the materials for Stage 2. ROCStories Corpora supplies a large quantity of pure textual
stories for generation in Stage 3, and the VIST Dataset, the sole end-to-end visual storytelling
dataset, helps fine-tune the model. Note that when we here refer to all
the available textual stories, these are from the VIST Dataset and the ROCStories Corpora. 

\paragraph{Visual Genome} 
Visual Genome contains labels for tasks in language and vision fields such as
object detection and object relation detection. 
Visual Genome has 108,077 images, 3.8 million object instances, and 2.3 million
relationships. We use it to pretrain the object detection model
used in Stage 1. In addition, we utilize the noun and verb relations provided by
the scene graph of Visual Genome to brainstorm activities which could link two
photos.   
Relations of nouns and verbs in each image have been labeled as \emph{(subject,
verb, object)}. 
The reasons we use verb relations are twofold. 
First, compared to unseen objects,
activities are better ingredients to add in visual stories for correlation
as they do less harm to grounding. Second, as most image-to-text datasets focus
on objects, stories generated based on them are relatively static. Hence adding
activities makes our stories vivid.  

\paragraph{OpenIE} 
OpenIE is an information extractor that finds relationships in 
sentences~\cite{pal2016demonyms,christensen2011analysis,saha2017bootstrapping,saha2018open}. 
Here we use its relations extracted from various corpora as another knowledge
base.\footnote{https://openie.allenai.org/}
Note that we only extract one-hop relations from OpenIE.

\paragraph{ROCStories Corpora} 
We use ROCStories, which contains 98,159 stories, to train the story
generator~\cite{mostafazadeh2016roc}. 
As the annotators of ROCStories were asked to write a five-sentence story given
a prompt, stories focus on a specific topic with strong logical inference.
Similar to VIST, we extract terms from sentences of stories which are used as
the input data of the story generation model.

\paragraph{VIST Dataset}
%\lwku{for plot term extraction \& finetune generated story} 
This is a collection of 20,211 human-written visual stories and 81,743 unique photos.
Each story in VIST contains five sentences and five corresponding photo images.
To train our image-to-term prediction model, we first extract terms from
sentences of stories in the VIST dataset as the gold labels.
Inspired by Semstyle~\cite{Alexander2018Semstyle}, we consider the key
components of the sentence to be its noun (object) and verb (action) terms;
therefore, given a sentence, we first detect nouns and verbs using a
part-of-speech tagger\footnote{SpaCy: https://spacy.io/}. Then, we extract verb
frames to replace original verbs using Open-SESAME~\cite{swayamdipta17open}, a
frame-semantic parser which automatically detects
FrameNet~\cite{baker1998berkeley} frames. For example, in
Table~\ref{tab:term_example}, the terms extracted from \textit{``The dog is ready to
go"} are ``Dog\_Noun" and ``Motion\_Frame".

As for the term-to-story generation model, the Transformer generator used in
Stage 3 is first trained on the ROCStories dataset with the textual stories and
their extracted terms, and then fine-tuned on both the ROCStories and VIST
datasets.


==> error_analysis.tex <==
\paragraph{Error Analysis}
To better understand the behavior of \system, we conduct a small-scale error analysis.
50 photo sequences and their corresponding stories are randomly selected and manually examined by one of the authors.
The following is the distribution of the error types.
%, and we categorize in which stage does the error happen.

\begin{enumerate}
    \item \textbf{Term Prediction Error (Stage 1): 44\%.}
    The term prediction error occurs when the story or terms are unrelated to the images content regardless the additional sentence. We find out that 44\% of the errors are of this type. The term that were unrelated to the images caused the model to generate irrelevant story, and thus, deteriorate the overall performance.
    \item \textbf{Relation Error (Stage 2): 26\%.}
    The relation error means the extracted relations are redundant with existing terms or does not match with visual content in the images. About 26\% of the stories were found to have relation error, however, this percentage is relatively small compared to the other two types of errors. Bounding the added relations with images may further mitigate their impact. 
    \item \textbf{Generation Error (Stage 3): 30\%.}
    Generation error refers to the low-quality generated sentence under the condition that the given terms are valid. 30\% of errors are of this type. This may result from some rarely seen combination of terms for which the generation model does not know how to describe them. Collecting a large quantity of diverse stories for learning could be a solution.
\end{enumerate}


==> experiment_result.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figure/case_study_v2.png}
	 \caption{Example stories generated by visual storytelling models. The knowledge-enriched sentences are highlighted.}
    \label{fig:case_study}
\end{figure*}

We conducted evaluations using both automatic
metrics and human ranking.
Automatic metrics were evaluated by shallow features such as the word coverage
or semantics for the quality stories~\cite{wang2018nometics}, whereas human
evaluation provided solid results due to their complete comprehension. 
For human evaluations, we adopted the ranking of stories from all models and the
stories written by humans. All human evaluations were conducted on the Amazon Mechanical Turk; five different workers were assigned for each comparison.
Through this direct comparison, we were able to provide a baseline for turkers,
yielding reliable results.
%\kenneth{this opening is pretty lengthy. Kenneth will shorten it later.}

% In human evaluation, two kinds of evaluation were performed: a standard rating evaluation and a direct comparison. 
% In the standard evaluation, annotators were asked to score the given story in terms of its \focus, \coherence, \shareability, \humanness, \grounding, and \detail, as in the Storytelling workshop~\cite{W18-1500}. 
% For the direct comparison evaluation, we provided the annotators with the stories generated by the different models, and asked them to rank these stories given and not given photos to study the visual attachment. 



% In human evaluation, two kinds of evaluation were performed: a standard rating evaluation and a direct comparison. 
% In the standard evaluation, annotators were asked to score the given story in terms of its \focus, \coherence, \shareability, \humanness, \grounding, and \detail, as in the Storytelling workshop~\cite{W18-1500}. 
% For the direct comparison evaluation, we provided the annotators with the stories generated by the different models, and asked them to rank these stories given and not given photos to study the visual attachment. 


\subsection{Human Evaluation}
%\subsubsection{Human Evaluation}

\input{figure/comparison_table.tex} 

\paragraph{Ranking Stories with Images}
We conducted a human evaluation using crowd workers recruited from Amazon
Mechanical Turk.
Each task displayed one sequence of photos and several generated stories based on
the sequence.
Five workers were recruited for each task to rank the story quality, ``from the
Best Story to the Worst Story.''
The compensation was \$0.10 per task.   % AMH: dollar amounts always use two significant digits
Four models were included in this evaluation: 
{\em (i)} \system using OpenIE as the knowledge graph,
{\em (ii)} \system using VisualGenome as the knowledge graph,
{\em (iii)} \system without any knowledge graphs, and {\em (iv)} GLAC~\cite{Kim2018GLACNG}, 
the current state-of-the-art visual storytelling model.
As we also included {\em (v)} human-written stories for comparison, the ranking
number is from 1 (the best) to 5 (the worst).
Table~\ref{tab:comparison} shows the evaluation results, showing that \system
benefits from the enrichment of knowledge. 
Stories generated by \system using either OpenIE or Visual Genome are on
average ranked significantly better (lower) than that of GLAC (unpaired t-test,
$p<0.05$, N = 2500), 
whereas stories generated by \system without using any knowledge graphs ranked
significantly worst (higher) (unpaired t-test, $p<0.01$, N = 2500).
%However, both models with knowledge graph fall behind humans' generated stories by about 0.13 in annotators' average ranks. 
%It means that there is still a large gap toward machine generating human-like stories.


\paragraph{Ranking Stories without Images}
\begin{table}[t]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{@{}lrrrrr@{}}
\multicolumn{6}{c}{Human Evaluation (Story Displayed \textbf{without} Images)} \\ \midrule
\textbf{} & \textbf{\begin{tabular}[c]{@{}r@{}}GLAC\\ \cite{Kim2018GLACNG}\end{tabular}} & \textbf{No KG} & \textbf{OpenIE} & \textbf{\begin{tabular}[c]{@{}r@{}}Visual\\ Genome\end{tabular}} & \textbf{Human} \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}Avg. Rank\\ (1 to 5)\end{tabular}} & 3.0538 & 3.2851 & \textbf{3.0492} & \textbf{2.9903} & 2.6210 \\ \bottomrule
\end{tabular}
}
\caption{Direct comparison evaluation without given photos. Numbers indicate average rank given to stories (from 1 to 5, lower is better).}
\label{tab:comparison-no-img}
\end{table}




We also explored the relation between images and the generated stories
in visual storytelling.
To determine whether the generated stories are well matched to the photos, we
removed the photos and conducted another overall story comparison. Results in
Table~\ref{tab:comparison-no-img} show that when
photos were provided in human evaluation, visual stories from the \system were
ranked higher than those from the state-of-the-art GLAC (2.97
vs. 3.05, significant with p-value $<$ 0.05); they become comparable (3.04 vs.
3.05) when the photos were not provided. The ranking of visual stories from the
state-of-the-art model remains the same. This
suggests that visual stories from \system better fit the photos, where
the images and texts support each other. 
The third story in   % AMH: second --> third
Figure~\ref{fig:case_study} illustrates an example. The visual story from
the state-of-the-art GLAC clearly is not grounded: there is no snow in
the second photo, no kids in the fourth, and no baby in the fifth, though
only considering the text it is a reasonable Christmas story. In contrast,
given the photos, the proposed \system generates an obviously better
story. This example also illustrates that the given images are both hints and
constraints in visual storytelling, which makes it a more challenging task than
general story generation. Besides, even when photos are not provided, the
average rank of visual stories from \system is comparable to that from the state-of-the-art
model. This demonstrates that our stories are both closely aligned to the
images and also stand without the images, which we attribute to the use
of the additional Virtual Genome dataset and ROCStories Corpora for the model
learning. 




\begin{comment}
 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figure/case_study.pdf}
	 \caption{Case Study. Italic sentences denote knowledge-graph-enriched sentences.}
    \label{fig:case_study}
\end{figure}
\end{comment}












\paragraph{The Effect of Using Knowledge Graphs}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figure/kg-analysis.png}
	 \caption{The distribution of the ranks received by each model. From the darkest blue to the lightest blue is the best rank to the worst.}
    \label{fig:histogram}
\end{figure}

We also investigate the effect of using a knowledge graph on story
quality.
Figure~\ref{fig:histogram} shows the distribution of ranks assigned to
models with and without the enrichment of the knowledge graph. Overall we note a clearly
increasing number of stories ranked as the first, second, and third
place when considering the knowledge graph, which confirms its
benefit to the quality of stories.
Specifically, stories from the model with the Visual Genome receive more first
ranks and also more worst ranks than those from the model with OpenIE. In
other words, compared to stories enriched by Virtual Genome, those from OpenIE
are relatively moderate. This may result from the existence of the two-hop
relations in Visual Genome, whereas OpenIE contains only one-hop relations. As a
result, the model with Visual Genome tends to be more imaginative and
unrestrained, leading to stories that are either extremely good or extremely
bad. 
%Furthermore, Figure \ref{fig:histogram} shows that model without knowledge graph receive more worst rank comparing to models with knowledge graph, prove again our model can benefit from the knowledge base integration.



\paragraph{Observing Automatic Metrics}

As prior work has clearly shown that the classic automatic evaluation metrics are
weak or even negative quality indicators for visual 
storytelling~\cite{hsu-etal-2019-visual,wang2018nometics}, we do not use these for
evaluation.
However, they still have something to say about token-based textual analysis.
Interestingly, we observe that the use of knowledge graphs increases the scores
in precision-based metrics (i.e., BLUE1, BLEU2, and CIDEr) with the cost of slightly
reduced scores in recall-based metrics (Table~\ref{tab:auto_eval}).
% This could be caused by the fact that \system looks for entities and their
% relations that are commonly mentioned by people; thus considering the knowledge
% graph and selecting tuples by the language model happens to help target the
% appropriate roles to enrich the story. The third story of   % AMH: again
% Figure~\ref{fig:case_study} also demonstrates this phenomenon. As a dog appears
% in both image (4) and (5), the human story includes it. In the OpenIE story,
% images (4) and (5) are successfully connected by the entity \textit{time} and
% \textit{dog}. However, the GLAC story selects another role \textit{kids} to
% tell and drafts \textit{baby} in the next sentence. \lwku{add the hit rate
% of entities and the added sentences.h}  


\input{table/auto_eval.tex}



%are obvious in the photos



%This could suggest that adding extra knowledge increases the precision of the generated tokens, with minor costs on token's recall.




\subsection{Discussion}



In this section, we discuss some of our observations throughout the
experiments.


\paragraph{A New Relation Bridges Two Images}
We observe that often the newly added relation creates bridges between two
images.
For example, for the first photo sequence in Figure~\ref{fig:case_study},
\system with Visual Genome distills \textit{friends} from the third image and
\textit{girls} from the fourth image.
Then the system connects the two terms with the two-hop relation \emph{(friends, posture,
man)} and \emph{(man, posture,
girls)}.
Similarly, \system with OpenIE links \emph{time} from the first image and \emph{everyone} from
the second image with the relation \emph{(time, cause to experience, everyone)}. 
We also find that after adding KG terms to the term set, the entire generated
story is different from the No-KG stories, even though the terms for the
original images are not changed. This shows that \system indeed considers all terms together when generating stories, and hence added terms influence its context.



\paragraph{Repetition Penalty Reduces Repetition}

We observe that there are repetitions in GLAC's stories. For example, in story ``\emph{the new office is a very interesting place. the kids love the toy. they also have a lot of books. they have a nice collection of books. they even have a stuffed animal}'' and ``\emph{the kids were having a great time at the party. they had a lot of fun. they had a lot of fun. they had a lot of fun. they had a great time.}'', 
the pattern ``\emph{they have}'' and ``\emph{they had a lot of fun}'' both respectively appear three times, which is generally less human and not ideal.
We find that this phenomenon is reduced by the repetition penalty in
\system.

\paragraph{When Nonexistent Entities Are Added}
Adding terms that refer to entities or people that are not actually in the
image is a potential risk when enriching stories with information from the KG. 
We find this problem to be especially severe for two-hop relations.
The second photo sequence in Figure~\ref{fig:case_study} is an example in which the
knowledge graph fails to help.
After \emph{building} is distilled from the second image and \emph{bridge} is distilled
from the third image, \system selects the link for enrichment: $\mathit{building}
\xrightarrow{\text{obscurity}} \mathit{bus} \xrightarrow{\text{travel}} \mathit{bridge}$.
While this link itself as well as the generated sentence ``\emph{there was a bus on
the bridge next to an old building}'' are both quite valid, it does not align
to the images as the bus, the building, and the bridge are not in the
described relative positions. 
In this case, the model generates unsatisfactory stories.

\input{error_analysis.tex}


\begin{comment}
By further investigating generated stories from the \system models,
the state-of-the-art SniBiVitt model, and turkers, we observe 
%some interesting phenomena. 
%First, 
that visual stories composed by turkers are sometimes boring and repetitive,
and hence are not good material for learning. 
For example, the second story in
Figure~\ref{fig:case_study} shows that annotators did not attempt to compose
a story connecting the photo sequence; instead they simply set down caption-like sentences.\kenneth{where is fig:case\_study}
In contrast, the enhanced \system(KB:scoring) successfully generates a
better story by leveraging additional data and knowledge.
\end{comment}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}



%


%=============== dead kitten ========================
 
\begin{comment}
 
 
either OpenIE or Visual Genome on average ranked higher than GLAC, while 

we also find that without the enhancement of knowledge graph, the \textbf{No KG} model is outperformed by the baseline model \textbf{GLAC}. 



Stories generated from three models, 

We evaluate three variants of the \system model using human evaluation.
One does not utilize any knowledge graph, another uses openIE as the knowledge graph and the other uses Visual Genome as the knowledge graph.

As shown in Table ~\ref{tab:comparison}, the human evaluation of both \system models with knowledge graph shows that they outperform the state-of-the-art.
And we also find that without the enhancement of knowledge graph, the \textbf{No KG} model is outperformed by the baseline model \textbf{GLAC}. 
Therefore we can conclude that our \system model benefits from the enrichment of knowledge. 
However, both models with knowledge graph fall behind humans' generated stories by about 0.13 in annotators' average ranks. 
It means that there is still a large gap toward machine generating human-like stories.


Instead of indicating

% =============== Kenneth is NOW working on auto eval ================

We also conduct classic automatic evaluation.
In Table~\ref{tab:auto_eval}, we report the experiment results of all models on five automatic evaluations (BLEU1, BLEU4, METEOR, ROUGE, CIDEr).
Results indicate our proposed methods (\textbf{OpenIE} and \textbf{Visual Genome}) generally outperform the baseline models. For BLEU1, both of our proposed method is about 20\% higher than the based line model. However, there is only slight difference in METEOR and ROUGE. 

Given BLUE and CIDEr are both precision-based metrics, we hypothesis that the additional knowledge our proposed model utilize can be also found in human generate stories. Therefore, the additional information of our stories convey can lead to the precision-based metrics increase. While KG provides apposite terms, the additional sentence enriches the story content, enhances the story continuity, and strengthens the sentence's coherence. 
Nevertheless, we note that literature \cite{hsu-etal-2019-visual} has suggested that automatic metric cannot evaluate storytelling properly.
In fact, these automatic metrics were originally designed for translation task, which is pretty different from our task.
Therefore we still need the result of human evaluation to judge which method can generate more human-satisfied stories.

%Note that comparing the KG story and No KG story,
 
\end{comment}

==> experiment_setup.tex <==
In this paper, \system leverages the
object detection model to find reliable candidates for story casting, which
provides robust grounding.
We also use the image knowledge graphs such as Visual
Genome~\cite{krishnavisualgenome} to extract activities to correlate the roles
selected by the system.
FrameNet~\cite{baker1998berkeley} terms are used to present the semantic
concepts of selected roles and their extracted correlated activities for the
story plot, which later guides the model to compose the visual story from a
panoramic point of view.
We describe the experimental setup in detail in this section.
%In experiment we show the superiority of \system for the visual storytelling task.
%Per human ranking evaluation, \system generates higher-quality stories than that of the state-of-the-art system.


\input{data.tex}

\subsection{Hyperparameter Configuration}
In all of our experiments, we used the same hyperparameters to train our model.
The hidden size of the term prediction and story generation models was set to
512. The head and layer number of the Transformer encoder were 2 and 4.
Both models
were trained with the Adam optimizer with an initial learning rate of 1e-3,
which decayed with the growth of training steps. 
During decoding, the beam size was set to 3 for both modules.


==> impact-automation.tex <==



%How did the automation impact the original Chorus workers?




%\kenneth{need to explain what is upvote and downvote}
%\subsection{Automating Human Labor}
During the deployment of \ev, a conversation on average contained 9.90 messages sent from the users, 
13.58 messages sent from the crowd workers, and 
1.93 messages sent from automatic chatterbots~\cite{Evorus}.
Thus, \textbf{automated responses were chosen 12.44\% of the time}.
As a comparison, without any automation, a conversation on average contained 8.73 user messages and 12.98 crowd messages.

%\paragraph{Conversation Quality}
In order to examine the conversation quality, we sampled conversations with accepted automatic responses and a matching set without automated contributions.
For each, 8 MTurk workers rated [Satisfaction, Clarity, Responsiveness, Comfort], which was based on the PARADISE's objectives for evaluating dialogue performance~\cite{paradise} and the Quality of Communication Experience metric~\cite{liu2010quality}, on a 5-point Likert scale (5 is best.)
The original conversations (N=46) had an average rating of [3.47, 4.04, 3.88, 3.56], while those with automatic responses (N=54) had [3.57, 3.74, 3.52, 3.66].
The similar results suggest that the automatic components did not make conversations worse. 






%\paragraph{Impact to Workers}


==> introduction.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/system_overview_v3.png}
    %\vspace{-5pc}
	 \caption{Overview of \system. \system first {\em (i)} distills a set of representative words from the input prompts and
{\em (ii)} enriches the word set by using external knowledge graphs, and
{\em (iii)} generates stories based on the enriched word set.}
    \label{fig:system}
\end{figure}

Stories are diverse and highly personalized.
Namely, story generation models, whether using text or images as input
prompts, aim at a large possible output space with rich information and
vocabulary.
One classic example is visual storytelling (VIST), an
interdisciplinary task that takes a sequence of five photos as the input and
generates a short story as the output~\cite{huang2016visual}.
However, existing visual storytelling approaches produce monotonous stories
with repetitive text and low lexical diversity~\cite{hsu-etal-2019-visual}.
We believe three major factors contribute to this problem.
%1.end-to-end single corpus
First, most prior work uses only a single training set ({\em i.e.},
the VIST dataset) in an end-to-end
manner~\cite{wang2018nometics,Kim2018GLACNG,wang2018show}.
Although this can result in legitimate stories, the end-to-end architecture
makes it difficult to use external data.
The generated stories are thus limited in terms of vocabulary and knowledge in VIST.
Similar phenomena are observed for text story generation models using a single
training set, where the output can be ``fairly generic''~\cite{fan2018hierarchical}.
%2. small data size
Second, the VIST dataset is considerably smaller than that of other text
generation tasks.
The MSCOCO dataset for image captioning contains 995,684
captions~\cite{lin2014microsoft};
the VQA dataset for visual question answering contains $\sim$0.76M questions
and $\sim$10M answers~\cite{antol2015vqa}; and the ROC dataset for text story
generation contains 98,159 stories~\cite{mostafazadeh2016roc}.
The VIST dataset, in contrast, contains only 49,603 stories.
Thus it is not surprising that stories generated using VIST show low lexical
diversity.
%3. no connection between images
Finally, no existing work takes into account relations between
photos.
Visual storytelling was introduced as an artificial intelligence task that attempts to
``interpret causal structure'' and ``make sense of visual input to tie
disparate moments together''~\cite{huang2016visual}.
However, existing approaches still treat it as a sequential image captioning
problem and omit relations between images.
%\kenneth{here should say something about KG used for video summary I guess?}







We introduce \system, a three-stage framework that allows the
story generation model to take advantage of external resources, especially
knowledge graphs, to produce interesting stories.
\system first distills a set of representative words from the input prompts and
enriches the word set using external knowledge graphs, and finally
generates stories based on the enriched word set.
This \textit{distill-enrich-generate} framework allows the use of external
resources not only for the enrichment phase, but also for the distillation and
generation phases.
%=============== 
Figure~\ref{fig:system} overviews the workflow of \system.
\system first distills a set of words from each image, respectively.
For example, the words {\tt Posture\_Frame} and {\tt graduates\_NOUN} are extracted from image (2), and the words {\tt Receiving\_Frame}, {\tt students\_NOUN} and {\tt diplomas\_NOUN} are extracted from image (3).
In stage 2, \system then searches in a knowledge graph to find potential relations between word pairs across images.
\system uses a scoring function to rate potential relations when multiple relations are found.
In Figure~\ref{fig:system}, the system finds the relation {\tt Arriving\_Frame} between {\tt graduates\_NOUN} and {\tt diplomas\_NOUN}, denoted as $\text{graduates\_NOUN} \xrightarrow{\text{Arriving\_Frame}} \text{diplomas\_NOUN}$.
Finally, in stage 3, \system uses an story generator to produce the final story sentence using all ingredients.
The {\tt Arriving\_Frame} is defined as ``An object Theme moves in the direction of a Goal.'' in the knowledge graph (FrameNet), illustrating a graduates' common body motion in the commencement. 
As a result, the phrase ``came out to take'' in the final output sentence captures this knowledge extracted by \system.

The system opens up possibilities to using large external data sources to improve
automated visual storytelling, instead of struggling with specialized small
data sources.
%end2end
%small data
%model relations between 










\begin{comment}



%In this paper, we opens up the possibilities of using these larger and more general external data to improve automated visual storytelling, instead of struggling with the specialized small data.



%open the opportunities of using larger and more general external data from these research outcomes to improve automated visual storytelling.



%------------- the followings are old text

%Inspired by the concept that editing prototypes benefits sentence
%generation~\cite{guu2018generating},  
We introduce \system, a two-stage visual storytelling model which separates the drafting of the
plot from the composition of the story text. This intermediate plot
disentangles image and text processing to facilitate data
utilization and knowledge acquisition.


% photos, where the former is in the vertical dimension (for each photo) while
% the latter is in the horizontal dimension (across photos), a two dimensional process. 
 We demonstrate that by dividing the task into two stages, we
are able to utilize large datasets of different modalities in different stages,
to produce an interpretable plot, and hence to add related ingredients to the
story. All these improve the quality of visual stories in terms of
\focus, \coherence, \shareability, \humanness, \grounding, and
\detail, and at the end yield the overall best story. 
\lwku{Now we only put on ranking results.....} 

We conduct two relatively large-scaled human evaluations compared to the VIST task, on
generated visual stories 
of 500 test photo sequences sampled from 1,000, 
by \system, the state-of-the-art model
SnuBiVtt~\cite{huang2016visual,kim2018glac} which performs best in VIST 2018, and turkers, respectively.
% Each visual story is
% evaluated from a total of seven aspects.
% , including six aspects in VIST standard
% evaluation: focus, coherence, shareability, humanness, grounding, detail, and entertainment, an
% additional aspect. 
% Results show that the proposed model composes
% the most entertaining and ``shareable'' visual stories..
% due to the good performance from the
% grounding, shareability, and entertainment aspects. 
Further case studies and an ablation experiment for the story's visual attachment are also included.




\kenneth{1. how many image-text pairs does MS COCO have? 2. how many img-text pairs does VQA have? 3. how many do VIST have? 4. how many stories do ROC have? Make a concrete comparison here. 3. Mention the size of KG you used here. Because that's the core part of the work.}
\zyc{1. MS COCO: 995684 caption for 164062 images. 2. VQA: ∼0.25M images, ∼0.76M questions, and ∼10M answers 3. VIST: 210819 photos and 49603 stories. 4. ROC:98159 stories }

Considering the relatively mature development of these similar research problems, reusing their datasets or models would be advantageous for visual storytelling. 

is an interdisciplinary task comprising image semantic reasoning and structural text generation, which takes a sequence of five photos as input and generates a short story for it.
As a result of using a single training set, 


As a result, 



even  was designed as an interdisciplinary task comprising image semantic reasoning and structural text generation,



was mostly done by 

resulting in a large possible output space for story generation.


, which result in a large possible output space for story generation task

as introduced by Huang et
al.~\cite{huang2016visual} in the VIST task, we take a sequence of photos as
input and attempt to
generate a short story narrating the sequence. 

This is an interdisciplinary task comprising image semantic reasoning and
structural text generation. 

Most previous models view this as an end-to-end
task~\cite{wang2018nometics,Kim2018GLACNG,wang2018show}.




Existing end-to-end approaches produce monotonous stories because they are limited to the vocabulary and knowledge in a single training dataset.
This paper introduces \textbf{\system}, a three-stage framework that allows the story generation model to take advantage of external \textbf{K}nowledge \textbf{G}raphs to produce interesting stories.
\system first {\em (i)} distills a set of representative words from the input prompts and
{\em (ii)} enriches the word set by using external knowledge graphs, and finally
{\em (iii)} generates stories based on the enriched word set.
This \textit{distill-enrich-generate} framework allows the use of external resources not only for enrichment phase, but also for distillation and generation phases.
In this paper, we show the superiority of \system in the visual storytelling task, where the input prompt is a sequence of five photos and the output is a short story.
Per human evaluation, \system generates higher-quality stories than that of the state-of-the-art system in nearly all aspects.


~\cite{fan2018hierarchical} 
%quote from the paper
In the generation of prompts using the GCNN
language model, we find that prompts are fairly
generic compared to human prompts. Language
models often struggle to model rare words accurately, as the probability distribution over the next
word is dominated by more common words. This
tends to produce similar prompts, particularly at
the start — we see many prompts that start with
the man. In contrast, many of the human prompts
are very unique (e.g. prompting stories in fantasy
worlds such as Harry Potter and Game of Thrones)
and the language model rarely produces the specific vocabulary required by these settings.


However, compared to the similar multi-modal research problem image
captioning task~\cite{lin2014microsoft} or uni-modal research question text
story generation~\cite{mostafazadeh2016roc}, the amount of its data for
end-to-end learning~\cite{huang2016visual} is limited, which
complicates the task. Considering the relatively mature development of these
similar research problems, reusing their datasets or models would be
advantageous for visual storytelling. 



%----------------- original intro -------------------------

In visual storytelling (VIST), as introduced by Huang et
al.~\cite{huang2016visual} in the VIST task, we take a sequence of photos as
input and attempt to
generate a short story narrating the sequence. 
This is an interdisciplinary task comprising image semantic reasoning and
structural text generation. Most previous models view this as an end-to-end
task~\cite{wang2018nometics,Kim2018GLACNG,wang2018show}.
However, compared to the similar multi-modal research problem image
captioning task~\cite{lin2014microsoft} or uni-modal research question text
story generation~\cite{mostafazadeh2016roc}, the amount of its data for
end-to-end learning~\cite{huang2016visual} is limited, which
complicates the task. Considering the relatively mature development of these
similar research problems, reusing their datasets or models would be
advantageous for visual storytelling. 

%Then a good option to utilize the small end-to-end dataset instead is for domain adaptation or style transformation in the learning process.
%
Another difference from image captioning~\cite{lin2014microsoft} is that authors
of visual stories can think up totally different stories for a given image
sequence based on their preference and imagination. Due to the large variety,
models learn to favor commonly seen sentences to avoid making mistakes, e.g.,
``they had a good time''. 
% In their reproduced
% results, we frequently observe sentences such as 
%``we are happy'' and 
Although these sentences are safe for composing different visual
stories, they are boring and trivial, as they carry little information. 
% Despite generating trivial sentences,
  In addition to their trivial nature,
caption-like sentences also destroy the storyline. Though this kind of sentence
mentions the most obvious objects in a photo, it is still uninteresting as it makes no
connections to other parts of the story. 
% For example, if there is a man in the first photo and a horse in the
% second, we have caption-like sentences such as ``There is a man in the park'' and
% ``There is a horse'', instead of ``A man is standing in the park'' and ``He is going
% to ride the horse''. 
A visual story consisting of caption-like sentences is not our goal,
much less what entertains us or what we would share with our friends. 

We attempt to compose a good visual story by enriching the
model learning process and the story generation process with data and
knowledge, respectively.
Inspired by the concept that editing prototypes benefits sentence
generation~\cite{guu2018generating},  
we introduce \system, a two-stage visual storytelling model which separates the drafting of the
plot from the composition of the story text. This intermediate plot
disentangles image and text processing to facilitate data
utilization and knowledge acquisition.


% photos, where the former is in the vertical dimension (for each photo) while
% the latter is in the horizontal dimension (across photos), a two dimensional process. 
Specifically, the model leverages the
object detection model to find reliable candidates for story casting,
which provides robust grounding. In addition, we utilize the image knowledge graph, i.e.,
the scene graph of Visual Genome~\cite{krishnavisualgenome}, to extract activities to correlate
the roles selected by \system. 
FrameNet~\cite{baker1998berkeley} terms are used to present the semantic
concepts of selected roles and their extracted correlated activities for the
story plot, which later guides the model to compose the visual story from a
panoramic point of view. We demonstrate that by dividing the task into two stages, we
are able to utilize large datasets of different modalities in different stages,
to produce an interpretable plot, and hence to add related ingredients to the
story. All these improve the quality of visual stories in terms of
\focus, \coherence, \shareability, \humanness, \grounding, and
\detail, and at the end yield the overall best story. 
%\lwku{explain later: relations are interactions which may not be recognized or revealed in photos.} 

We conduct two relatively large-scaled human evaluations compared to the VIST task, on
generated visual stories 
of 500 test photo sequences sampled from 1,000, 
by \system, the state-of-the-art model
SnuBiVtt~\cite{huang2016visual,kim2018glac} which performs best in VIST 2018, and turkers, respectively.
% Each visual story is
% evaluated from a total of seven aspects.
% , including six aspects in VIST standard
% evaluation: focus, coherence, shareability, humanness, grounding, detail, and entertainment, an
% additional aspect. 
% Results show that the proposed model composes
% the most entertaining and ``shareable'' visual stories..
% due to the good performance from the
% grounding, shareability, and entertainment aspects. 
Further case studies and an ablation experiment for the story's visual attachment are also included.


%Beyond understanding simple objects and concrete scenes lies interpreting causal structure; 
%making sense of visual input to tie disparate moments together as they give rise to a cohesive %narrative of events through time. 


This requires moving from reasoning about single images – static moments, devoid of context – to sequences of images that depict
events as they occur and change. On the vision side,
progressing from single images to images in context
allows us to begin to create an artificial intelligence
(AI) that can reason about a visual moment given

what it has already seen. On the language side, progressing from literal description to narrative helps to
learn more evaluative, conversational, and abstract
language. This is the difference between, for example, “sitting next to each other” versus “having
a good time”, or “sun is setting” versus “sky illuminated with a brilliance...” (see Figure 1). The first
descriptions capture image content that is literal and
concrete; the second requires further inference about
what a good time may look like, or what is special
and worth sharing about a particular sunset.



%Then a good option to utilize the small end-to-end dataset instead is for domain adaptation or style transformation in the learning process.
%
Another difference from image captioning~\cite{lin2014microsoft} is that authors
of visual stories can think up totally different stories for a given image
sequence based on their preference and imagination. Due to the large variety,
models learn to favor commonly seen sentences to avoid making mistakes, e.g.,
``they had a good time''. 
% In their reproduced
% results, we frequently observe sentences such as 
%``we are happy'' and 
Although these sentences are safe for composing different visual
stories, they are boring and trivial, as they carry little information. 
% Despite generating trivial sentences,
  In addition to their trivial nature,
caption-like sentences also destroy the storyline. Though this kind of sentence
mentions the most obvious objects in a photo, it is still uninteresting as it makes no
connections to other parts of the story. 
% For example, if there is a man in the first photo and a horse in the
% second, we have caption-like sentences such as ``There is a man in the park'' and
% ``There is a horse'', instead of ``A man is standing in the park'' and ``He is going
% to ride the horse''. 
A visual story consisting of caption-like sentences is not our goal,
much less what entertains us or what we would share with our friends. 









%One further disadvantage of the single-corpus approach is the size of data.


\end{comment}

==> related_work.tex <==


%~\cite{Wang2019HierarchicalPE,Kim2018GLACNG,wang2018nometics,Kim2018GLACNG,wang2018show}

%\paragraph{Multi-Stage Story Generation}
%Recent studies have been done on two-stage text story generation.
As researchers have found that middle-level abstraction can result in more
coherent stories,~\cite{yao2019plan} show that more diverse stories are
generated by using a pipeline involving first planning the overall storyline
and then composing the story.
They propose an event-based method which transforms the previous story into
event representations, predicts successive events, and generates a story using
the predicted events~\cite{martin2018event}.
Similarly,~\cite{xu2018skeleton} propose a skeleton-based narrative story
generation method which uses a skeleton as a middle-level abstraction layer.
However, 
%these techniques are rarely applied in visual storytelling. %perhaps it could be explored further.
%\paragraph{Multi-Stage Visual Storytelling}
although multi-stage text story generation has been a focus of recent studies,
limited effort has been expended on multi-stage visual storytelling.
%due to the challenge posed by its multi-modal nature. 
One of the few exceptions is work done
by Huang et al.~\shortcite{DBLP:journals/corr/abs-1805-08191}.
Leveraging the middle-level abstraction as well, they propose a two-level
hierarchical decoder model for the VIST task.
They first predict a topic ({\em e.g.}, indoors, kids, the baby) for each image
in the sequence, after which the low-level decoder generates a sentence for each image
conditioned on the given topic.
The two decoders are jointly trained end-to-end using reinforcement learning.
As the topics can be selected only from fixed clusters using a discriminative
model, the ability of story planning is limited. 
Furthermore, under an end-to-end training process, extra plain text and knowledge
base data cannot be utilized to better enrich the story.
In a similar task,~\cite{Alexander2018Semstyle} propose a two-stage style
transfer model for image captioning.
Their first stage consists of keyword prediction for the caption of each
independent image, and then a stylish caption is generated using an RNN trained
on story corpora.
However, each such caption is a single story-like sentence and is independent
of other captions; combined, the captions do not constitute a context-coherent
story.






==> system.tex <==
%distill-enrich-generate

%\begin{figure}[!t]
%   \centering
%    \includegraphics[width=1\col%umnwidth]{figure/model_arch.pdf}
%    \caption{Model architecture %of \system \kenneth{now we have %3 stages. please update the %chart accordingly.}}
%    \label{fig:model_arch}
%    
%\end{figure}






In this work, a three-stage approach is proposed for knowledge-enriched visual
storytelling.

\begin{description}
    \item[Stage 1: Word distillation from input prompts.]
	 Given a sequence of images, we train an image-to-term model to distill
	 terms from each of the input images; this can be regarded as word-form conceptual representation.
    \item[Stage 2: Word enrichment using knowledge graphs.]
	 With the five sets of terms extracted in the previous step, we utilize an external
	 knowledge graph to identify possible links between sets, and generate the
	 final enriched term path for story generation. 
    \item[Stage 3: Story generation.]
	 We use a Transformer architecture to transform term paths into stories. A
	 length-difference positional encoding and a repetition penalty are used in
	 the proposed Transformer; we also apply a novel anaphoric expression
	 generator.
\end{description}

In the following, we describe the three steps in detail.





\subsection{Stage 1: Word Distillation from Input Prompts}
%\subsection{Step 1: Distill Words from Input Prompts}

\begin{figure}[t]
    \centering
    \includegraphics[
    %trim=4cm 10cm 1.5cm 3cm,
    width=1\columnwidth]{figure/step1.pdf}

	 \caption{Stage 1: Image distillation model. In Stage 1, \system extract terms from the image. To this end, we build a model that uses a pre-trained Faster R-CNN as the image encoder and a Transformer-GRU as the term decoder.}

    \label{fig:step1}
\end{figure}

In Stage 1, we extract terms from the image. To this end, we build a model that uses a pre-trained Faster R-CNN~\cite{ren2015faster,anderson2018bottom} as the image encoder and a Transformer-GRU as the term decoder.

The Faster R-CNN model was originally trained for the object detection task. Here we extract the features of its predicted object as the image representation. To reduce computational complexity, only the object features within the top 25 confidence scores are used.

As shown in Figure~\ref{fig:step1}, the image representation is fed into a Transformer encoder~\cite{vaswani2017attention} and a GRU~\cite{chung2014empirical} decoder with an attention mechanism~\cite{bahdanau2014neural} as our term prediction model.
%to generate terms from object features of every image. 
%The terms is a simplified version of sentence that contains the key information such as object and actions and will be used to construct a whole story in the following stage.
The only modification to the Transformer for distillation is the positional encoding.
In contrast to the positional encoding in the original setting, object
features are summed with trainable image-order embeddings as input, as
objects in the same image are sequentially independent:
\begin{align*}
x_i = Wo_i + \text{Order\_Embedding}(t)
\end{align*}
where $o_i$ is the $i$-th object and $t$ is the order of the image.
$W^{2048\times D}$ is a matrix that transforms the 2048-dimensional $o_i$ into
dimension $D$.
Then object features are fed into the term prediction model to generate the
terms for each photo.
%To avoid redundant terms, we apply a repetition penalty to terms that have appeared in previous photos.
During decoding, we use an intra-sentence repetition penalty with beam
search to reduce redundancy in the visual story~\cite{hsu2018using}. 
The term score at each beam search step is computed as
\begin{align*}
\mbox{beam\_score}(x) = \log(p(x))-1e^{19}\cdot\mathds{1}(x{\in}S),
\end{align*}
where $p(x)$ is the model's output probability for each term, the last term
denotes repetition penalty, and set $S$ denotes terms that have already been
predicted in an image.




\subsection{Stage 2: Word Enrichment Using Knowledge Graphs}
Given a sequence of images for story generation, we have observed that nearly 
irrelevant sequential images are common.
In previous end-to-end models, such a phenomenon hurts story generation and causes
models to create caption-like incoherent stories which are relatively boring
and semantically disconnected.
To take this into account while enriching the story, we introduce
semantic terms as the intermediate and link terms in two adjacent images using
the relations provided by the knowledge graph.
%, which not only leads to the possibility of using non-end-to-end training data, but also brings the opportunity to solve the low-related sequential images issue.
%We solve this issue by extract possible path the starts with a term in previous image and end with a term the next image in a knowledge base. 
In the knowledge graph, real world knowledge is encoded by entities and their
relationship in the form of tuples \emph{(head, rela, tail)}, indicating that
\emph{head} has a \emph{rela} relationship with \emph{tail}. 

More specifically, given all the terms predicted in the previous step $\{m^1_{1},
.., m^t_i, .. ,m^5_{N_5}\}$, where $m^t_i$ denotes the $i$-th term distilled
from the $t$-th image, we pair the terms from two consecutive images and
query the knowledge graph for all possible tuples $\{...., (m^t_i, r_k,
m^{t+1}_j), ....\}$ where $r_k$ is a one-hop relation that links $m^t_i$ and
$m^{t+1}_j$ in the knowledge graph.
Furthermore, we also consider two-hop relations, which can convey indirect
relationships, to enrich the story by adding $(m^t_i, r_k, m_{\mathit{middle}}, r_q,
m^{t+1}_j)$ if such a relation exists in the knowledge graph.

After all tuples of one- and two-hop relations are extracted, we 
construct candidate terms from them and insert each relation into the term set
for story generation, i.e., the extracted $(m^l_i, r_k, m^{l+1}_j)$ or
$(m^l_i, r_k, m_{\mathit{middle}}, r_q, m^{l+1}_j)$, which contains the head term from image
$l$ and the tail term from image ${l+1}$, is inserted between images $l$ and
${l+1}$ to generate an additional story sentence, 
as if these were the terms distilled in between the images.   % AMH: check

With all possible term sets constructed, we must select the most reasonable
one for the next term-to-story generation step.
Hence we train an RNN-based language model on all the available textual stories. 
A language model estimates the probability distribution of a corpus
$$ P(U) = \Sigma \text{logP}(u_i|u_{1},...,u{i-1}) $$
where $U = {u_1, ..., u_n}$ is the corpus.
Here we use it to compute the probability of a term conditioned on the other
terms existing previously.
Thus we obtain the perplexity of this term path, choose that term path with the
lowest perplexity, and feed it to the next step.

Actually, Stage 2 mimics the way people generate a story based on two
irrelevant images, that is, relating two images through imagination. Here the
knowledge graph serves as the source of ideas connecting two images and the
language model then ensures the coherence of the generated story when using the
selected idea.












\subsection{Step 3: Story Generation}

\begin{figure}[t]
    \centering
    \includegraphics[
    %trim=4cm 10cm 1.5cm 3cm,
    width=1\columnwidth]{figure/step3.pdf}
	 \caption{Stage 3: Story generation model. For the story generation step, we leverage
the Transformer with the input ({\em i.e.}, the term set) from Stage 2. }

    \label{fig:step3}
\end{figure}

For the story generation step, we leverage
the Transformer~\cite{vaswani2017attention} shown in Figure~\ref{fig:step3} with the
input, i.e., the term set, from Stage 2. 
We add to the original Transformer model three different modifications:
{\em (i)} length-difference positional encoding for variable-length story generation,
{\em (ii)} anaphoric expression generation for the unification of anaphor representation,
and {\em (iii)} a repetition penalty for removing redundancy.

\paragraph{Length-Difference Positional Encoding}
The sinusoidal positional encoding method~\cite{vaswani2017attention} inserts
the absolute positions to a sinusoidal function to create a positional
embedding. However, when the model is used to generate variable-length stories,
this positional encoding method makes it difficult for the model to recognize
sentence position in a story. For the visual storytelling task, all the
samples contain five images, each of which is described generally in one sentence
for the corresponding storyline; thus the generated stories always contain five sentences, which
prevents us from adding additional ingredients to enrich them. To tackle this
problem, we adopt length-difference positional encoding
(LDPE)~\cite{Takase_2019} as shown in Equations~(\ref{eqn:LDPE1}) and
(\ref{eqn:LDPE2}), where $\mathit{pos}$ is the position, $d$ is the embedding
size, $\mathit{len}$ is the length constraint, $i$ is the dimension of the sinusoidal
positional encoding, and ${10000^{2i/d}} \times {2}$ is the period of a
sinusoidal function. 
LDPE allows the Transformer to learn positional embeddings with variable-length stories.
Unlike positional encoding that uses absolute positions, LDPE
returns the remaining length of a story. As a result, the terminal position is
identical for dissimilar story lengths. Consequently, the model learns to
generate ending sentence for stories with different lengths.
\begin{equation}
\label{eqn:LDPE1}
\mathit{LDPE}_{(\mathit{pos},\mathit{len},2i)} = \sin \biggl(\frac{\mathit{len}-\mathit{pos}}{10000^{\frac{2i}{d}}}\biggr)
\end{equation}

\begin{equation}
\label{eqn:LDPE2}
\mathit{LDPE}_{(\mathit{pos},\mathit{len},2i+1)} = \cos \biggl(\frac{\mathit{len}-\mathit{pos}}{10000^{\frac{2i}{d}}}\biggr)
\end{equation}



\paragraph{Anaphoric Expression Generation}
To enable the use of pronouns in the enhanced \system model for anaphoric
expression generation, we adopt a coreference replacement strategy.
%The use of pronoun will cause the mismatch between two modules in our system. Pronouns in a story are used to refer the entities that participants in the story or be mentioned elsewhere in the story. An entity that appears multiple times in a photo sequence will be detected repetitively, but a story depicting the photo sequence should use pronoun to replace the entity. 
% As shown in Table~\ref{tab:term_example}, the short visual story of two successive images that both contain a dog, and the corresponding story is \textit{"The dog is ready to go. He is playing on the ground."} Without coreference replacement, the term predictor will learn to predict "dog" term for both images while the story generator cannot learn that since its training input does not have "dog" term for the second sentence. %For term predictor model, the gold label of both images have the “dog” term, but the input data for story generation model will not have “dog” for the second sentece.
%To deal with this mismatch, we utilize coreference replacement. 
To replace coreferences, we first use a coreference
resolution tool\footnote{NeuralCoref 4.0: Coreference Resolution in spaCy with Neural Networks. https://github.com/huggingface/neuralcoref}
on the stories to find the original mention of each pronoun and replace the
pronouns with their root entities. The entity types are the ten defined in the
OntoNotes dataset~\cite{weischedel2013ontonotes}, including PERSON,
PRODUCT, ORG, and so on. Open-SESAME then extracts terms again from the 
stories in which the coreferences have been replaced; 
these extracted terms are then used as the input~-- 
with the original stories as the output~-- to train the story generator
in Stage 2. As such, the story generator learns to generate pronouns given
two successive identical noun terms. Table~\ref{tab:term_example} shows a
short visual story of two successive images where both contain the same
object (a dog), and the corresponding gold story reads ``\emph{The dog is ready to
go. He is playing on the ground.}'' In this example, the term predictor 
predicts \emph{dog} for both images, but the term extractor cannot extract
\emph{dog} from the second gold sentence. To bridge this gap, coreference
replacement replaces the pronoun with its original mention ``\emph{the dog}'' in the second
gold sentence, which enables the story generator to learn to generate anaphoric
expressions when seeing multiple mentions of ``\emph{the dog}''.

\input{table/coreference.tex}  % tab:term_example

\paragraph{Repetition Penalty in Story Generation}
Instead of using a repetition penalty for predicted terms only, we use inter- and
intra-sentence repetition penalties with beam search to reduce redundancy in the
visual story~\cite{hsu2018using}. The word score at each beam search step is
\begin{align*}
\mbox{beam\_score}(x) = \log(p(x))-\alpha\cdot\mathds{1}(x{\in}S)\\-(\gamma/l)\cdot\mathds{1}(x{\in}R),
\end{align*}
where $\alpha$ and $\gamma$ are hyperparameters empirically set to 20 and
5. Set $S$ denotes words that appear in the current sentence, and set $R$
denotes words in previous sentences. The current story's length $l$
is a regularization term which reduces the penalty to prevent the story
generator from refusing to repeat words when generating grammatically
correct sentences as the length of the sentence or story increases.

\begin{comment}

For Step 3 story generation, we leverage
Transformer~\cite{vaswani2017attention} shown in Figure~\ref{fig:step3} with the
input, i.e., the term set, from Step 2. 

Three different modifications, including length-difference positional encoding for various-length story generation, anaphoric expression generation for the unification of anaphor representation, and repetition penalty for removing redundancy, were added to the original Transformer model.

\paragraph{Length-Difference Positional Encoding}
The sinusoidal positional encoding method~\cite{vaswani2017attention} inserts the absolute positions to a sinusoidal function to create a positional embedding. However, when the model is generating stories with various lengths, this positional encoding method causes difficulties for the model to recognize sentence position in a story. For the visual storytelling task, as all the samples contain 5 images and for each the corresponding storyline is described mostly in one sentence, the generated stories always contain 5 sentences, which prevents us from adding additional ingredients to enrich them. To tackle this problem, we adopt length-difference positional encoding (LDPE)~\cite{Takase_2019} as shown in Equation~ (\ref{eqn:LDPE1}) and Equation~(\ref{eqn:LDPE2}), where $pos$ is the position, $d$ is the embedding size, $len$ is the length constraint, $i$ is the dimension of the sinusoidal positional encoding, and ${10000^{2i/d}} \times {2}$ is the period of a sinusoidal function. 
LPDE allows Transformer to learn positional embedding with various story lengths. Unlike positional encoding that is using absolute positions, LDPE returns the remaining length of a story. As a result, the terminal position is identical for dissimilar story lengths. Consequently, the model learns to generate ending sentence for stories with different lengths.
\begin{equation}
\label{eqn:LDPE1}
LDPE_{(pos,len,2i)} = sin \biggl(\frac{len-pos}{10000^{\frac{2i}{d}}}\biggr)
\end{equation}

\begin{equation}
\label{eqn:LDPE2}
LDPE_{(pos,len,2i+1)} = cos \biggl(\frac{len-pos}{10000^{\frac{2i}{d}}}\biggr)
\end{equation}



\paragraph{Anaphoric Expression Generation}
To enable the use of pronouns in the enhanced \system model for anaphoric
expression generation, we adopt a coreference replacement strategy.
%The use of pronoun will cause the mismatch between two modules in our system. Pronouns in a story are used to refer the entities that participants in the story or be mentioned elsewhere in the story. An entity that appears multiple times in a photo sequence will be detected repetitively, but a story depicting the photo sequence should use pronoun to replace the entity. 
% As shown in Table~\ref{tab:term_example}, the short visual story of two successive images that both contain a dog, and the corresponding story is \textit{"The dog is ready to go. He is playing on the ground."} Without coreference replacement, the term predictor will learn to predict "dog" term for both images while the story generator cannot learn that since its training input does not have "dog" term for the second sentence. %For term predictor model, the gold label of both images have the “dog” term, but the input data for story generation model will not have “dog” for the second sentece.
%To deal with this mismatch, we utilize coreference replacement. 
To replace coreferences, we first use a coreference
resolution tool\footnote{https://github.com/huggingface/neuralcoref} 
on the stories to find the original mention of each pronoun and replace the
pronouns with their root entities. The entity types are the 10 defined in the
OntoNotes dataset~\cite{weischedel2013ontonotes}, including ``PERSON'',
``PRODUCT'', ``ORG'', and so on. Open-SESAME then extracts terms again from the 
stories in which the coreferences have been replaced; 
these extracted terms are then used as the input~-- 
with the original stories as the output~-- to train the story generator
in stage two. As such, the story generator learns to generate pronouns given
two successive identical noun terms. Table~\ref{tab:term_example} shows an
short visual story of two successive images where both contain the same
object (a dog), and the corresponding gold story reads \emph{``The dog is ready to
go. He is playing on the ground.''} In this example, the term predictor 
predicts \emph{dog} for both images, but the term extractor cannot extract
\emph{dog} from the second gold sentence. To bridge this gap, coreference
replacement replaces the pronoun with its original mention ``the dog'' in the second
gold sentence, which enables the story generator to learn to generate anaphoric
expressions when seeing multiple mentions of ``the dog''.

\input{table/coreference.tex}  % tab:term_example

\paragraph{Repetition Penalty in Story Generation}
Instead of using a repetition penalty only on predicted terms, we use inter- and
intra-sentence repetition penalties with beam search to reduce redundancy in the
visual story~\cite{hsu2018using}. The word score at each beam search step is
\begin{align*}
\mbox{beam\_score}(x) = \log(p(x))-\alpha\cdot\mathds{1}(x{\in}S)\\-(\gamma/l)\cdot\mathds{1}(x{\in}R),
\end{align*}
where $\alpha$ and $\gamma$ are hyperparameters empirically set to 20 and
5. Set $S$ denotes words that appear in the current sentence, and set $R$
denotes words in previous sentences. The current story's length $l$
is a regularization term which reduces the penalty to prevent the story
generator from refusing to repeat words when generating grammatically
correct sentences as the length of the sentence or story increases.


%=======================
\end{comment}


==> table/auto_eval.tex <==
\begin{comment}

\begin{table}[htbp]
\tiny
\begin{tabular}{@{}llllllll@{}}
              & BLEU\_1 & BLEU\_2 & BLEU\_3 & BLEU\_4 & METEOR & ROUGE\_L & CIDEr \\ \midrule
GLAC      & .374   & .185   & .093   & .050   & .297  & .250    & .049 \\
No KG        & .376   & .185   & .096   & .050   & .295  & .237    & .055 \\
OpenIE        & .446   & .223   & .109   & .056   & .297  & .241    & .094 \\
VisualGenome & .451   & .223   & .109   & .056   & .296  & .241    & .096 \\ \bottomrule
\end{tabular}
\caption{\small Comparison for four models on seven kinds of automatic evaluation.}
\end{table}

\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htbp]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{@{}lrrrrr@{}}
\toprule
 & \textbf{BLEU1} & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{CIDEr} \\ \midrule
\textbf{GLAC~\cite{Kim2018GLACNG}} & .374 & .050 & \textbf{.297} & \textbf{.250} & .049 \\ \midrule
\textbf{No KG} & .376 & .050 & .295 & .237 & .055 \\
\textbf{OpenIE} & .446 & \textbf{.056} & \textbf{.297} & .241 & .094 \\
\textbf{Visual Genome} & \textbf{.451} & \textbf{.056} & .296 & .241 & \textbf{.096} \\ \bottomrule
\end{tabular}
}
\caption{Automatic evaluation results. Prior work has clearly shown that the classic automatic evaluation metrics are
weak or even negative quality indicators for visual 
storytelling~\cite{hsu-etal-2019-visual,wang2018nometics}.}
\label{tab:auto_eval}
\end{table}



==> table/coreference.tex <==
\begin{table}[]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l|l|l}
 &\includegraphics[width=0.17\textwidth]{figure/dog1.jpg}
 &\includegraphics[width=0.17\textwidth]{figure/dog2.jpg} \\ \hline
\begin{tabular}[c]{@{}l@{}}Original \\ story\end{tabular} & \begin{tabular}[c]{@{}l@{}}The dog is\\  ready to go.\end{tabular} & \begin{tabular}[c]{@{}l@{}}He is playing \\ on the ground.\end{tabular}      \\ \hline
Terms                                                     & \begin{tabular}[c]{@{}l@{}}``Dog\_Noun'',\\  ``Motion\_Frame''\end{tabular}             & \begin{tabular}[c]{@{}l@{}}``Performers\_and\_roles\_Frame'',\\ ``Ground\_Noun''\end{tabular}                   \\ \hline\hline
\begin{tabular}[c]{@{}l@{}}Story \\ w/ CR\end{tabular}    & \begin{tabular}[c]{@{}l@{}}The dog is \\ ready to go.\end{tabular} & \begin{tabular}[c]{@{}l@{}}The dog is playing \\ on the ground.\end{tabular} \\ \hline 
Terms                                                     & \begin{tabular}[c]{@{}l@{}}``Dog\_Noun'',\\ ``Motion\_Frame''\end{tabular}             & \begin{tabular}[c]{@{}l@{}}``Dog\_Noun'',\\ ``Performers\_and\_roles\_Frame'',\\  ``Ground\_Noun''\end{tabular}           \\ \hline
\end{tabular}
}
\caption{Term extraction and coreference replacement (CR). Image
order is from left to right.}
\label{tab:term_example}
\end{table}


==> table/error_analysis.tex <==
\begin{table}[]
\begin{tabular}{l|l}
                             & Story \\ \hline
Grounded Error               & 22    \\
Relation Error               & 13    \\
Model Story Generation Error & 15  
\label{tab:error_analysis_1}
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{ll}
        & Grounded Error                                                                                                                                                                 \\ \hline
Example & OpenIE: we went to a museum today . the room was very old . we had a great time there . the band went on for a long time . the band played music . then we came back to town . \\
Cons    & There is no museum in the images                                                                                                                                     \label{tab:error_analysis_2}
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{ll}
        & Relation Error                                                                                                                                                                 \\ \hline
Visual Genome: i went to the city today . there were many people gathered to watch . when i got there they looked like a zebra food . it was a lot of good food . everyone had a great time . the crowd was very big .\\
Cons    & The object generated by Visual Genome: zebra is not in the images.                                                                                             \label{tab:error_analysis_3}
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{ll}
        & Model Story Generation Error                                                                                                                                                                 \\ \hline
17398173-17399304-17399712-17400033-17401748-
Visual Genome: the family got together for dinner . the food was very tasty . we put some food in a napkin as well . the main dish was delicious . we ate it all . we had a lot of drinks .\\
Cons    & The images are related to restaurant, so it's reasonable to have napkins in the term set.  However, the model generates "we put some food in a napkin as well", which use the napkins to construct an inappropriate sentence.                                                                                             \label{tab:error_analysis_3}
\end{tabular}
\end{table}

==> table/standard_comparison.tex <==
\begin{table}[!ht]
\centering
\small
%\resizebox{0.8\textwidth}{!}{
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
%Team & Focused & Coherent & Shareable & Human & Grounded & Detailed & Entertaining  \\
 & F & C & S & H & G & D   \\
\midrule
Human & 3.64 & 3.47 & 3.19 & 3.45 & 3.59 & 3.49 \\
\midrule
SnuBiVtt & 3.18	& 3.00	& 2.82	& 2.86	& 2.78	& 2.80  \\
\midrule\midrule

Enhanced PlotVist\\
\midrule
%\begin{tabular}[c]{@{}l@{}}$\text{PlotVIST}^{\text{1+}}$\end{tabular}
\begin{tabular}[c]{@{}l@{}}$\hspace{3mm}\text{-w/o KB}$\end{tabular}
& \textbf{3.22} & \textbf{3.24} & \textbf{3.21} & \textbf{3.27} & 3.25 & 3.24  \\

\begin{tabular}[c]{@{}l@{}}$\hspace{3mm}\text{-w/ KB: random}$\end{tabular} & 3.08 & 3.14 & 3.15 & 3.16 & \textbf{3.28} & \textbf{3.30} \\

\begin{tabular}[c]{@{}l@{}}$\hspace{3mm}\text{-w/ KB: scoring}$\end{tabular} & 3.21 & 3.13 & 3.11 & 3.13 & 3.12 & 3.11 \\ 
\midrule


\end{tabular}
}

\caption{\small Standard rating evaluation for Improved \system for six categories:
\focus (F), \coherence (C), \shareability (S), \humanness (H), \grounding (G), and \detail (D).}

\label{tab:emnlp-standard}

\end{table}


==> table/with_or_without_image_comparison_table.tex <==



% \begin{table}[!ht]
% \centering
% \small
% \resizebox{1\columnwidth}{!}{

% \begin{tabular}{ccccc}
% \toprule
%   & Human & SnuBiVtt & Basic PlotVist & $\text{PlotVist}^{\text{ w/o KB}}$ \\
%   %& $\text{P}^{\text{2+}}$ \\
% \midrule
% Overall & 2.04 & 3.18 & 3.34 & 3.28 \\
% %& \textbf{3.16}  \\
% % \midrule
% % Entertaining & 2.20 & 3.21 & 3.41 & 3.13 & \textbf{3.06} \\
% \midrule
% $\text{Overall}^-$ & 2.15 & \textbf{2.76} & 3.34 & 3.34 \\
% %& 3.41 \\
% \midrule 

% \end{tabular}
% }

% \caption{\small Direct comparison evaluation for the basic \system model. Numbers indicate average rank given to stories (from 1 to 5, lower is better).}
% \label{tab:comp_result_basic}

% \end{table}


\begin{table}[!ht]
\centering
\small
\resizebox{1\columnwidth}{!}{


\begin{tabular}{cccccc}
\toprule
  & Human & SnuBiVtt & $\text{P}^{\text{ w/o KB}}$ & $\text{P}^{\text{ random}}$ & $\text{P}^{\text{ scoring}}$ \\
\midrule
Overall & 2.42 & 3.16 & 3.42 & 3.02 & \textbf{2.98}  \\
% \midrule
% Entertaining & 2.33 & 3.19 & 3.46 & 3.02 & \textbf{3.00} \\
\midrule
$\text{Overall}^-$ & 2.55 & \textbf{2.98} & 3.32 & 3.11 & 3.04 \\
\midrule 

\end{tabular}
}

\caption{\small Direct comparison evaluation for the enhanced \system model.
Numbers indicate average rank given to stories (from 1 to 5, lower is better).}
\label{tab:comp_result_improved}

\end{table}


